villa-X: Enhancing Latent Action Modeling in Vision-Language-Action Models

Vision-Language-Action (VLA) models have emerged as a popular paradigm for learning robot manipulation policies that can follow language instructions and generalize to novel scenarios. Recent works have begun to explore the incorporation of latent actions, abstract representations of motion between two frames, into VLA pre-training. In this paper, we introduce villa-X, a novel Vision-Language-Latent-Action (ViLLA) framework that advances latent action modeling for learning generalizable robot manipulation policies. Our approach improves both how latent actions are learned and how they are incorporated into VLA pre-training. We demonstrate that villa-X can generate latent action plans in a zero-shot fashion, even for unseen embodiments and open-vocabulary symbolic understanding. This capability enables villa-X to achieve superior performance across diverse simulation tasks in SIMPLER and on two real-world robotic setups involving both gripper and dexterous hand manipulation. These results establish villa-X as a principled and scalable paradigm for learning generalizable robot manipulation policies. We believe it provides a strong foundation for future research.

==> sections/conclusion.tex <==
\section{Conclusion, Limitations, and Future Works}

In this paper, we presented villa-X, a novel Visual-Language-Latent-Action (ViLLA) framework that improves both the learning of latent actions and their incorporation into VLA pre-training. Our experiments demonstrate that our enhanced Latent Action Model learns higher-quality latent actions, and our improved policy model more effectively leverages these learned actions. Overall, our method exhibits superior performance in both simulated environments and real-world robotic tasks.

One limitation is that the proposed latent expert, although effective at future planning through both visual and proprioceptive state planning, is not fully explored in this work. For example, future research could learn a critic with prior knowledge from foundation vision-language models, allowing multiple samples from the latent expert and rejecting planned trajectories that do not follow the language instruction. We leave this aspect as future work to further improve the capability of the ViLLA framework.

==> sections/experiment.tex <==

\section{Experiments}

In this section, we aim to answer the following questions through experiments:
\begin{itemize}[left=10pt]
\item Does our improved \lam\ learn higher-quality latent actions?
\item Can \texttt{ACT-latent} successfully plan future motions?
\item Can the actor module effectively leverage the pre-trained latent actions?
\item How does \methodname\ compare to existing VLA baselines in both simulated benchmarks and real-world robot tasks?
\end{itemize}

\subsection{Does our improved \lam\ learn higher-quality latent actions?}
\label{sec:exp-lam}

In this subsection, we evaluate whether our improved latent action modeling enhances the quality of the learned latent actions.
The key component of our \lam is the incorporation of the proprio FDM module.
To assess its impact, we compare our model (denoted \texttt{w/pp}) to a variant without the proprio FDM module (denoted \texttt{wo/pp}).


\textbf{Probing} \quad First, a core expectation for latent actions is that they should carry information useful for predicting low-level robot actions.
To test this, we conduct a probing experiment.
Specifically, after training the latent action models, we freeze them and train a simple 3-layer MLP to predict the corresponding robot actions for each latent action.
Probing is conducted on the LIBERO dataset~\cite{liu2023libero}, which is not used for training latent action models.
We train the MLP on the training split of LIBERO and evaluate it using the L1 loss on the validation split.

\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
    \vspace{-15pt}  % optional: adjust vertical position
    \includegraphics[width=0.4\textwidth]{figs/probing.png}
    \caption{Probing experiment results.}
    \label{fig:probing}
    \vspace{-15pt}  % optional: reduce space after figure
\end{wrapfigure}

We are interested in how closely the predicted actions match the ground truth.
In LIBERO, the robot action space has 8 dimensions: 3 for position, 4 for rotation, and 1 for the gripper.
Rather than averaging the error across dimensions, we focus on the maximum L1 error across all action dimensions, as we want to avoid large deviations in any single aspect of the action.
For each model variant (\texttt{w/pp} and \texttt{wo/pp}), we compute the number of validation samples whose maximum L1 error falls below a threshold.
By sweeping this threshold, we count how many samples fall within each error bin.
A better model should yield more samples with low errors.


For each error bin, we compute the difference in the number of samples between the \texttt{w/pp} and \texttt{wo/pp} variants and present the results in Figure~\ref{fig:probing}.
The \texttt{w/pp} variant produces more samples with smaller errors, while the \texttt{wo/pp} variant has more samples in the high-error bins.
This demonstrates the effectiveness of the proprio FDM module in capturing information from the robot actions.

\begin{table}[t]
    \centering
    \caption{Evaluation results on SIMPLER for different variants of our \methodname (top group) and alternative approaches for incorporating latent actions (bottom group).
    "Ours" refers to the \texttt{w/pp} described in the main text.}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{lcccccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{Google robot}} & \multicolumn{5}{c}{\textbf{WidowX robot}} \\
        \cmidrule(lr){2-6} \cmidrule(lr){7-11}
         & \makecell{\small{Pick}} & \makecell{\small{Move}} & \makecell{\small{Drawer}} & \makecell{\small{Place}} & \small{Avg.} & \makecell{\small{Carrot}} & \makecell{\small{Eggplant}} & \makecell{\small{Spoon}} & \makecell{\small{Cube}} & \small{Avg.} \\ 
        \midrule
        Ours & \textbf{81.7} & \textbf{55.4} & 38.4 & 4.2 & \textbf{44.9} & 24.2 & \textbf{71.7} & \textbf{48.3} & \textbf{19.2} & \textbf{40.8} \\
        \midrule
        \texttt{wo/pp} & 77.0 & 52.7 & \textbf{42.6} & 2.8 & 43.8 & 22.5 & 57.5 & 43.3 & 5.9 & 32.3 \\
        \texttt{wo/LAM} & 42.1 & 24.6 & 38.4 & 0.0 & 26.3 & \textbf{25.8} & 60.8 & 36.7 & 9.2 & 33.1 \\
        \midrule
        LAPA-style & 64.7 & 28.8 & 38.0 & \textbf{5.6} & 34.2 & 0.8 & 0.0 & 2.5 & 0.8 & 1.0 \\
        Go-1-style & 29.0 & 38.0 & 31.3 & 4.6 & 25.7 & 5.8 & 50.8 & 1.7 & 1.0 & 14.8 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:ablate-lam-simpler}
\end{table}

\textbf{Policy Pre-training} \quad
Next, we compare how the latent actions generated by different variants of \lam (\texttt{w/pp} and \texttt{wo/pp}) influence policy pre-training.
{Unlike the main experiments, we pretrain models in this section}
on a mixture of 10\% Fractal~\cite{brohan2022rt1} data, 10\% Bridge V2~\cite{ebert2021bridge} data, and 100\% Something-Something V2~\cite{goyal2017something} data, 
{to reduce computation cost while remaining a setting where limited robot data are available for training the VLA model.}
The resulting policies are evaluated in the SIMPLER environment~\cite{li2024evaluating}, a simulation benchmark explicitly designed to mitigate the gap between simulated and real‐world robotic environments. It comprises two platforms, namely Google robot and WidowX robot, each with four manipulation tasks. We evaluate our method on all the 8 tasks on the visual matching setting.
The results are summarized in Table~\ref{tab:ablate-lam-simpler}.
We observe that \texttt{w/pp} clearly outperforms \texttt{wo/pp}, demonstrating the effectiveness of incorporating the proprio FDM module.
Additionally, we include a baseline that does not use latent actions (denoted \texttt{wo/LAM}) and is trained solely to predict robot actions.
The performance of \texttt{wo/LAM} is significantly worse, indicating that pre-training with latent actions is essential.


\paragraph{LAM visualization} Figure \ref{fig:lam-visualization} visualizes image pairs sharing the same latent action, demonstrating that these pairs correspond to similar underlying robot behaviors.
To further demonstrate the transfer ability of our \texttt{LAM}, we extract latent actions from arbitrary video sequences, map them to robot actions using the proprio FDM, and execute the resulting robot action in SIMPLER simulator. 
The simulated motions closely reproduce the original demonstrations, indicating that latent actions are both aligned with and grounded in the robot’s actions. For more examples, please check Appendix \ref{appC:similar_la}.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/WM_transfer1.png}
    \caption{Transfer of human demonstrations to new scenes via latent actions and a world model. (a) moving right. (b) moving downwards. Please visit \href{https://aka.ms/villa-x}{our website} for more demos.}
    \label{fig:wm_transfer}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/Sim_transfer1.png}
    \caption{Transfer of video demonstrations into robot action executions via latent actions and a proprio FDM. Please visit \href{https://aka.ms/villa-x}{our website} for more demos.}
    \label{fig:sim_transfer}
\end{figure}

\paragraph{LAM transfer consistency} We provide two visualizations to further evaluate the transfer consistency of the learned latent actions. Specifically, we first use the trained LAM to extract a sequence of latent actions from a source video. These latent actions are then applied to different initial images, allowing a world model to generate subsequent frames conditioned on these actions.
As shown in Figure \ref{fig:wm_transfer}, the transfer rollouts (highlighted in blue) successfully identify the movable parts and demonstrate behaviors consistent with the original video. 


We also evaluate the alignment between latent and robot actions. To do this, we use the proprio FDM to decode latent actions into executable robot actions. These actions are then executed in the SIMPLER simulator, with the resulting rollouts visualized in Figure~\ref{fig:sim_transfer}.
In each example, the top row shows the original video demonstration from which latent actions were extracted, while the bottom row displays the corresponding simulated execution. The simulated motions closely match the original demonstrations, confirming that the latent actions learned by \methodname are well-aligned with and grounded in the robot actions.

\subsection{Can \texttt{ACT-latent} successfully plan future motions?}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/latent_expert_wm.pdf}
    \caption{Transfer of video demonstrations into robot action executions via latent actions and a proprio FDM. Please visit \href{https://aka.ms/villa-x}{our website} for more demos.}
    \vspace{-10pt}
    \label{fig:latent_expert_wm}
\end{figure}

In this experiment, we demostrate the motion planning capabilities of \texttt{ACT-latent} by visualizing its planned actions with a world model. For a given initial image and language instruction, \texttt{ACT-latent} generates a sequence of latent actions, and the world model takes the inital frame and latent actions as inputs to render the latent actions into planned future videos. Figure~\ref{fig:latent_expert_wm} shows results for both in-distribution and out-of-distribution samples, where the in-distribution samples are randomly sampled from the validation set but from the same datasets as used in training, and the out-of-distribution samples are from new real-world scenarios. The results demonstrate that \texttt{ACT-latent} successfully follows the language instructions to solve the tasks, while accurately identifying target objects and generating latent actions that successfully follow the instructions. \texttt{ACT-latent} also successfully identifies the concepts in the emoji, which rarely appears in robot datasets, suggesting that \methodname keeps the general vision-language capabilities in the initial VLM model after pre-training. 



\subsection{Can the actor module effectively leverage the pre-trained latent actions?}
\label{sec:exp-policy}

Given high-quality latent actions produced by the pre-trained \lam, we investigate whether our design can effectively leverage them to pre-train robot control policies.
We compare our approach against two recent methods that also utilize latent actions, albeit in different ways: LAPA~\cite{ye2024latent} and GO-1~\cite{agibot-world-contributors2025agibot}. 

To isolate the effect of how latent actions are incorporated, we implement LAPA-style and GO-1-style models based on our architecture for a fair comparison.
For the LAPA-style model, we follow a two-stage pre-training protocol: we first train the VLM to predict latent actions, then replace the latent action prediction head with a robot action prediction head and continue training on data with robot action labels.
For the GO-1-style model, we implement a separate latent planner that autoregressively predicts latent actions.
The robot action prediction component remains largely unchanged as in our main design.

Following the experiment setup in the previous subsection, we train all models on the same dataset mixture and then evaluate the resulting policies in the SIMPLER environment~\cite{li2024evaluating}.
The results are shown in Table~\ref{tab:ablate-lam-simpler}.
Compared to other two approaches, our method achieves significantly higher performance, validating the effectiveness of our design for incorporating latent actions into VLA pre-training.


\subsection{Evaluating \methodname in Simulation}

\subsubsection{SIMPLER Benchmark}


\begin{table}[t]
    \centering
    \caption{Comparison on SIMPLER of \methodname and existing methods. Methods marked with $*$ are evaluated directly after pretraining, whereas other methods are evaluated after post-training on corresponding dataset. }
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{lccccccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{Google Robot}} & & \multicolumn{5}{c}{\textbf{WidowX Robot}} \\
        % \noalign{\vskip 3pt}
        \cline{2-6} \cline{8-12}
        % \noalign{\vskip 3pt}
         & \makecell{\small{Pick}} & \makecell{\small{Move}} & \makecell{\small{Drawer}} & \makecell{\small{Place}} & \small{Avg.} & & \makecell{\small{Carrot}} & \makecell{\small{Eggplant}} & \makecell{\small{Spoon}} & \makecell{\small{Cube}} & \small{Avg.}. \\ 
        \midrule
        RT-1-X $*$ & 56.7 & 31.7 & \textbf{59.7} & 21.3 & 42.4 & & 4.2 & 0.0 & 0.0 & 0.0 & 1.1 \\
        Octo-base $*$  & 17.0 & 4.2 & 22.7 & 0.0 & 11.0 & & 8.3 & 43.1 & 12.5 & 0.0 & 16.0 \\
        OpenVLA $*$ & 16.3 & 46.2 & 35.6 & 0.0 & 24.5 & & 0.0 & 4.1 & 0.0 & 0.0 & 1.0\\
        RoboVLMs $*$ & 72.7 & 66.3 & 26.8 & \textbf{36.1} & 50.5 & & 25.0 & 0.0 & 20.8 & 8.3 & 13.5\\
        RoboVLMs & 77.3 & 61.7 & 43.5 & 24.1 & 51.7 & & 20.8 & \textbf{79.2} & 45.8 & 4.2 & 37.5 \\
        % \midrule
        GR00T-N1.5 & 69.3 & 68.7 & 35.8 & 4.0 & 44.5 & & \textbf{54.3} & 61.3 & 75.3 & 57.0 & 62.0 \\
        % GR00T & 0.7 & 1.9  & 2.9 & 0.0 & 1.4 & & 0.0 & 13.9 & 1.4 & 0.0 & 3.8 \\
        MoTo & 74.0 & 60.4 & 43.1 & \texttt{N/A} & \texttt{N/A} & & \texttt{N/A} & \texttt{N/A} & \texttt{N/A} & \texttt{N/A} & \texttt{N/A}\\
        LAPA & \texttt{N/A} & \texttt{N/A} & \texttt{N/A} & \texttt{N/A} & \texttt{N/A} & & 45.8 & 58.3 & 70.8 & 54.2 & 57.3 \\
        \midrule
        \textbf{Ours} \small{w/o latent} & 56.3 & 25.8 & 27.3 & 13.9 & 30.8  & & 31.3 & 74.6 & 61.7 & 28.3 & 49.0\\
        \textbf{Ours} & \textbf{98.7} & \textbf{75.0} & \textbf{59.3} & 5.6 & \textbf{59.6} & & 46.3 & 64.6 & \textbf{77.9} & \textbf{61.3} & \textbf{62.5}\\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:results-simpler}
\end{table}

\paragraph{Baselines and Experimental Setup} We use the SIMPLER benchmark as described above. In this section, we compare against two categories of prior work:
\begin{itemize}[left=10pt]
    \item Vision-Language-Action (VLA) models: RT-1-X~\cite{open_x_embodiment_rt_x_2023}, Octo-base~\cite{octo_2023}, OpenVLA~\cite{kim2024openvla}, RoboVLMs~\cite{li2023generalist}, which learn policies solely from mixed robot datasets.
    \item Joint policy learning and world modeling method: GR00T-N1.5 ~\cite{nvidia2025gr00tn1openfoundation}, which aligns the model with target future embeddings.
    \item Latent-Action based methods: MoTo \cite{chen2024moto} and LAPA~\cite{ye2024latent}, which additionally exploit unlabelled videos by inferring latent actions.
\end{itemize}
Except where noted ($*$), all models follow a two‐stage pretraining–finetuning protocol, including a general pretraining phase on large‐scale mixed data, followed by finetuning on a dataset of specific embodiment. We also include an ablation (\methodname{} w/o latent) that removes our latent‐action expert while keeping all other components unchanged. Reported baseline scores are taken directly from the original publications, while missing entries are marked as \texttt{N/A}.

\paragraph{Experimental Results} Table \ref{tab:results-simpler} summarizes the success rates on both platforms. Our full model achieves the highest score on average success rate on the Google robot ($59.6$\%) and the WidowX robot ($62.5$\%). 
This improvement over VLA methods, which cannot exploit unlabelled video, demonstrates the benefit of our incorporating human videos into policy learning. Moreover, our approach outperforms other latent‐action methods, indicating that our specific mechanism for leveraging video data is more effective. Finally, the gap between our full model and the “\methodname{} w/o latent” ablation confirms that the latent‐action expert is essential for achieving these gains.



\subsubsection{LIBERO Benchmark}
The LIBERO benchmark~\cite{liu2023libero} evaluates knowledge transfer in multitask and lifelong robot learning problems for robotic manipulation, consisting of four task suites: \textbf{LIBERO-Spatial} evaluates the model's performance under novel layouts with the same task and object types,
\textbf{LIBERO-Goal} evaluates the model's performance under novel tasks with the same object types and layouts, 
\textbf{LIBERO-Object} evaluates the model's performance under novel object types with the same tasks and layouts,  
\textbf{LIBERO-Long} evaluates the model's performance under diverse set of objects, layouts and backgrounds. Each task suite contains 10 tasks with 50 human demonstrations per task for fine-tuning. 

\paragraph{Baselines and Experimental Setup} We compare with the following existing models: Diffusion Policy~\cite{chi2023diffusion} trained from scratch, Octo~\cite{octo_2023}, and OpenVLA~\cite{kim2024openvla}. 
All models follow a two-stage pretraining-finetuning protocol.
We finetune \methodname and \methodname w/o latent on the demonstration data of the each task suite separately, and test on the LIBERO simulator for 10 tasks and 20 trials per task on each task suite. 

\paragraph{Experimental Results} Table \ref{tab:results-libero} summarizes the success rates on each task suite of LIBERO. Our model achieves better performance than existing methods in all the four task suites. Also, our model with latent action achieves higher performance on 3 of the 4 task suites and average performance, confirming that the proposed latent action expert improves the manipulation performance. 


\iffalse 

\begin{table}[ht]
    \centering
    \caption{Results on CALVIN (ABC -> D)}
    \begin{tabular}{cccccccc}
        \toprule
         \multirow{2}{*}{Method} & \multirow{2}{*}{Input} & \multicolumn{6}{c}{Tasks competed in a row (1000 chains)} \\
         \cmidrule{3-8}
         & & 1 & 2 & 3 & 4 & 5 & Avg. Len. \\
         \midrule
         GR-1~\cite{wu2023unleashing} & S-RGB + G-RGB + P & 0.854 & 0.712 & 0.596 & 0.497 & 0.401 & 3.06 \\
         CogAct~\cite{li2024cogact} & S-RGB & 0.XX & 0.XX & 0.XX & 0.XX & 0.XX & xx \\
         GR00T~\cite{nvidia2025gr00t} & S-RGB & 0.XX & 0.XX & 0.XX & 0.XX & 0.XX & xx \\
         Moto~\cite{chen2024moto} & S-RGB & 0.897 & 0.729 & 0.601 & 0.484 & 0.386 & 3.10 \\
         Dita~\cite{hou2025dita0} & S-RGB & 0.945 & 0.825 & 0.728 & 0.613 & 0.500 & 3.61 \\
        \midrule
        \methodname & S-RGB & 0.XX & 0.XX & 0.XX & 0.XX & 0.XX & xx \\
        \bottomrule
    \end{tabular}
    \label{tab:results-calvin}
\end{table}

\fi


\begin{table}[ht]
    \centering
    \caption{Evaluation on 4 LIBERO task suites of \methodname and existing methods.
    }
    \begin{adjustbox}{width=0.68\textwidth}
    
    \begin{tabular}{lcccccc}
        \toprule
        Method & Spatial & Object & Goal & Long & Average \\
        \midrule
        Diffusion Policy~\cite{chi2023diffusion} & 78.3 & 92.5 & 68.3 & 50.5 & 72.4 \\
        Octo-base~\cite{octo_2023} & 78.9 & 85.7 & 84.6 & 51.1 & 75.1 \\
        OpenVLA~\cite{kim2024openvla} & 84.7 & 88.4 & 79.2 & 53.7 & 76.5 \\
        \midrule
        \textbf{Ours} \small{w/o latent} & 86.0 & 86.5 & 85.0 & 70.0 & 81.9 \\
        \textbf{Ours} & \textbf{97.5} &  \textbf{97.0} & \textbf{91.5} & \textbf{74.5} & \textbf{90.1} & \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:results-libero}
\end{table}

\subsection{Evaluating \methodname on Real-world Robots}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/real_robot.png}
    \caption{Real-world robot evaluation platforms: \textbf{(top)} Realman robot arm platform with a gripper and \textbf{(bottom)} Xarm robot arm with Xhand dexterous hand. Platform setups are shown on the left, with corresponding evaluation tasks on the right.
    Please visit \href{https://aka.ms/villa-x}{our website} for more videos.}
    \label{fig:xhand_env}
\end{figure}

\begin{table}[t]
    \centering
    \caption{Evaluation on Xarm robot arm of \methodname and existing methods.
    }
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{lcccccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}}  & \multicolumn{2}{c}{Pick \& Place} & \multicolumn{2}{c}{Stack Cube}
               & \multicolumn{2}{c}{Place Cup Upright} & \multicolumn{2}{c}{Pour Water}
               & \multicolumn{2}{c}{Flick Ball} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
               & seen & unseen & seen & unseen & seen & unseen & seen & unseen & seen & unseen \\
        \midrule
        GR-1                     & 56 & 40 & 15 & 5  & 0  & 0  & 0  & 0  & 40 & 10 \\
        GR00T                    & 44 & 28 & 20 & 0  & 20 & 0  & 0  & 0  & 30 & 0  \\
        \textbf{Ours} \small{w/o latent} & 72 & 60 & 70 & 40 & 40 & 30 & 40 & 10 & 50 & 30 \\
        \textbf{Ours}            & \textbf{84} & \textbf{68} & \textbf{75} & \textbf{50} & \textbf{60} & \textbf{30} & \textbf{60} & \textbf{30} & \textbf{50} & \textbf{40} \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:results-xhand}
\end{table}

\begin{table}[t]
    \centering
    \caption{Evaluation on Realman robot arm of \methodname and existing methods.
    }
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{lcccccccccc}
        \toprule
        \textbf{Method} & Pick in & Pick out & Push & Stack & Unstack & Change block color & Change table cover \\
        \midrule
GR00T                    & 30 & 70  & 10 & 10 & 60  & 50 & 30 \\
\textbf{Ours} \small{w/o latent} & \textbf{40} & 80  & 30 & \textbf{60} & 70  & 40 & 30 \\
\textbf{Ours}                     & 30 & \textbf{100} & \textbf{50} & 50 & \textbf{100} & \textbf{60} & \textbf{60} \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:results-realman}
\end{table}

To further assess generalization, we evaluate our approach on two real‑world robotic platforms: a Realman robot arm with a gripper, and an Xarm manipulator equipped with a 12‑DOF Xhand dexterous hand. See Figure \ref{fig:xhand_env} for details.

\paragraph{Realman robot arm with gripper} 
On the robot-arm manipulation platform, we use a 6-DoF Realman RM 75 robot arm and a 1-DoF Inspire gripper. 
We fine-tune and evaluate our policy on ``Pick-in'' (pick the block into a bowl), ``Pick-out'' (pick the block out of a bowl), ``Stack'' (stack the block onto another block), ``Unstack'' (unstack the block from another block), and ``Push'' (push the block to a given location) tasks.
For fine-tuning, we collect a dataset of 375 trajectories through teleoperation (with 75 trajectories for each task), where the object layout and table setup are fixed and only the object locations are dynamic.

We conduct two sets of evaluation: 
In task evaluation, we remain the table setup the same as data collection; 
in generalization evaluation, we change the color of the block and table cover. We evaluate the policy with 10 trials per task with each trial conducted with different object location, where all the experiment settings are the same for the evaluation of different policies (including the object location and lightening condition). 
The results are shown in Table \ref{tab:results-realman}, demonstrating that \methodname outperforms existing baselines in both task and generalization evaluation sets.

\paragraph{Xarm robot arm with Xhand dexterous hand} 

On the dexterous‑hand platform, we use the Xhand, a 12‑DoF dexterous hand with five flexible fingers, mounted on a 7-DoF Xarm robot arm.
Fine‑tuning is performed on the Xhand Dataset \cite{hu2024video}, which comprises 4,000 trajectories spanning 13 task categories. 
Since no dexterous-hand data were used during pretraining, this evaluation can test embodiment transfer ability.
We select five representative tasks—pick‑and‑place, cube stacking, cup upright placement, water pouring and ball flicking.
The results are summarized in Table \ref{tab:results-xhand} for (i) seen tasks, where objects are randomly replaced or additional distractors are added, and (ii) unseen tasks, which use unseen objects or backgrounds. The performances are evaluated under 50 runs for pick and place, 20 runs for stack cube and 10 runs for others.
Table \ref{tab:results-xhand} demonstrates that our method outperforms existing baselines.


==> sections/intro.tex <==
\section{Introduction}

Latent action learning has emerged as a promising approach for the pretraining of vision-language-action (VLA) models~\cite{black2024pi0,li2024cogact,nvidia2025gr00t,chen2024moto,kim2024openvla,zhao2025cot0vla0,xinghang2024vision,open_x_embodiment_rt_x_2023}, enabling learning from both robot data and human video data~\cite{ye2024latent,chen2024moto,nvidia2025gr00t,agibot-world-contributors2025agibot}.
At the core of these methods is a Latent Action Model (LAM), which compresses visual changes between successive frames into latent tokens, referred to as latent actions.
These latent actions are expected to capture motion semantics.
These tokens function as pseudo-action labels for imitation learning and enriching robot policy training with abundant, action-free data.


Yet two questions remain: \textit{how to learn latent actions} and \textit{how to incorporate latent actions into VLA pre-training}?
In this paper, we introduce \methodname{}, a novel Visual-Language-Latent-Action (ViLLA) framework that advances both key aspects of latent action modeling.
For the latent action learning component, a key limitation is the absence of direct alignment between visual transitions and underlying robot states and actions.
Although robot data with low-level states and actions are often available alongside action-free videos during pretraining, current methods choose to ignore these signals and focus solely on the visual part.
As a result, latent actions can remain ungrounded in the robot’s physical dynamics, resulting in a weak correspondence between latent action and robot behavior.
To address this issue, we incorporate a proprio Forward Dynamics Model (FDM) module into the LAM as an auxiliary decoder.
This module predicts future robot proprioceptive states and actions, encouraging the learned latent actions to better reflect the agent's behavior—not just the observed visual changes.
Moreover, this design improves the interpretability of the learned latent actions and enables them to be more easily translated into executable robot actions.
As a result, latent actions become a robust intermediary between vision-based representations and low-level controls. To exploit this structure, we propose to model the latent action and robot action distribution jointly through a joint diffusion process, and conditioning robot action generation on latent actions generation through attention.
Compared to existing methods on latent action pre-training, our approach allows for more effective and structured information transfer from latent actions to robot actions.


We conduct comprehensive evaluations of \methodname{} on two simulated environments, SIMPLER and LIBERO, as well as two real-world setups, including various robot platforms with gripper and dexterous hand manipulation. Our results demonstrate that \methodname{} achieves superior performance, laying a robust foundation for future research in this domain. 

Our contributions are listed as follows:
\begin{itemize}
    \item  We improve latent action learning by introducing an extra proprio FDM, which aligns latent tokens with underlying robot states and actions and grounds them in physical dynamics.
    \item We propose to jointly learn a latent action expert and a robot action expert through joint diffusion in the policy model, conditioning robot action prediction on latent actions to fully exploit their potential.
    \item Our method demonstrates superior performance on simulated environments as well as on real-world robotic tasks. The latent action expert can effectively plan into future with both visual and proprio state planning. 
\end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/overview.png}
    \caption{(a) High-level architecture of our \methodname method. (b) Detailed structure of the Latent Action Model (LAM) component within \methodname.}
    \label{fig:overview}
\end{figure}


==> sections/method.tex <==
\section{Method}
\label{sec:method}



\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/la_cluster_demo.pdf}
    \caption{Visualization of image pairs with similar latent actions.
    }
    \label{fig:lam-visualization}
\end{figure}


At a high level, our \methodname consists of two main components, as illustrated in Figure~\ref{fig:overview}a:
\begin{enumerate}[label=(\roman*)]
    \item a \texttt{LAM} (Latent Action Model) module that infers latent actions from a pair of observations;
    \item a \texttt{ACT} (Actor) module that jointly models latent actions and robot actions given an initial visual observation and a textual task instruction.
\end{enumerate}
We describe each component in detail in the following subsections.
Learning in \methodname is carried out in three stages:
(1) pretraining the \texttt{LAM} module,
(2) pretraining the \texttt{ACT} module, and
(3) finetuning \texttt{ACT} on target-embodiment data.


\subsection{Latent Action Model}
\label{sec:method-lam}


Modeling latent actions enables the use of abundant action-free video demonstration data and also holds the promise of improving generalization between robot and human motions~\cite{ye2024latent, chen2024moto}.
Building on these prior works, our \texttt{LAM} (depicted in Figure~\ref{fig:overview}b) learns an inverse dynamics model (IDM) to extract latent actions $z_t$ from two adjacent video frames, $o_t$ and $o_{t+K}$.
The interval $K$ is a configurable window size, chosen to balance perceptibility and generalizability: large enough to capture meaningful motion but small enough to maintain transferability.


Previous works~\cite{ye2024latent, chen2024moto} train IDM by jointly optimizing a forward dynamics model (FDM) to predict future frames.
Given the current frame $o_t$ and a latent action $z_t$, the model minimizes the discrepancy between the predicted frame $\hat{o}_{t+K}$ and the ground truth $o_{t+K}$.
Although robot data with low-level states and actions are often available alongside action-free video data, these approaches completely discards such information, focusing solely on visual changes.
Since our ultimate objective is to use latent actions to facilitate real robots policy learning, bridging vision-language prompts and low-level controls would be beneficial. To this end, we propose augmenting \texttt{LAM} pretraining with proprioceptive supervision.
Specifically, since $z_t$ represents a higher-level action abstraction, we introduce an additional proprio FDM module that predicts future robot states and actions $K$ steps ahead given the current robot state $q_t$ and the latent action $z_t$. This alignment of high-level abstractions and physical robot dynamics enhances the suitability of latent action for robot policy learning.

However, because robot trajectories are often embodiment specific, conditioning solely on $q_t$ and $z_t$ may embed platform-dependent features in the latent action, hindering cross-embodiment transfer.
To alleviate this issue, we provide the proprio FDM with an additional embodiment context input (\eg, dataset ID, control frequency),
isolating transferable action representations from embodiment particulars.


\paragraph{\includegraphics[height=8pt]{figs/gear.png} Implementation}
In practice, instead of predicting a single latent action between two frames (as Figure~\ref{fig:overview}b depicts), LAM receives a sequence of $T_{\text{LAM}}$ observation frames as input and outputs $T_{\text{LAM}} - 1$ latent actions between consecutive frames. The inverse dynamics model first encodes the frame sequence with a Spatial–Temporal Transformer~\cite{xu2020spatial0temporal}, then applies value quantization to produce $T_{\text{LAM}} - 1$ latent actions $z \in \mathbb{R}^{N_z \times D_d}$.
The FDM is implemented using a Vision Transformer (ViT), while the proprio FDM is a two-layer MLP with dual output heads.
The embodiment context input is embedded using learnable embeddings and concatenated with the robot state before being fed into the proprio FDM.
For further implementation details and configuration specifics, please refer to the appendix.

\paragraph{\textnormal{\PaperPortrait}~Training and Inference}

We train \texttt{LAM} on diverse data sources, including robot trajectories and human egocentric videos.
For data lacking low-level state and action labels, we omit the proprio FDM branch and optimize only the FDM reconstruction loss.
By leveraging this diverse data, our goal is to learn a generalizable intermediate representation for downstream policy learning.
Once trained, only the IDM is required to extract latent actions from a pair of frames at inference, the FDM and proprioceptive FDM serve primarily as diagnostic visualization tools. We use a mixture of datasets containing both human video and robot action data including OpenX \cite{open_x_embodiment_rt_x_2023}, Ego4D \cite{Ego4D2022CVPR}, etc. For more details, please refer to Appendix \ref{appA:lam_model}.

\subsection{Actor Module}
\label{sec:method-act}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/act.png}
    \caption{Structure of the \texttt{ACT} module.}
    \label{fig:act}
\end{figure}

In the same vein as common VLA models~\cite{kim2024openvla,li2024cogact,black2024pi0,ye2024latent,nvidia2025gr00t}, our \texttt{ACT} module builds upon a pre-trained vision-language model (VLM) and is trained to model a generalizable robot control policy that outputs actions given a textual task instruction and an initial observation.
With the pre-trained \texttt{LAM}, 
we are able to incorporate latent actions as an additional intermediate representation in our framework, rather than directly mapping vision and language inputs to low-level robot actions.
The latent actions serve as a bridging language that connects task prompts to robot action planning.

Figure~\ref{fig:act} provides an illustration of our \texttt{ACT} module, which consists of three components: VLM, \texttt{ACT-latent}, and \texttt{ACT-robot}.
Given a textual task prompt $l$ and a visual observation $o_t$, the VLM first extracts visual and language features.
Then, the \texttt{ACT-latent} component, trained with a diffusion objective, models a sequence of $n$ latent actions $z_t, z_{t+K}, \ldots, z_{t+(n-1)K}$, conditioned on the features from the VLM.
Subsequently, the \texttt{ACT-robot} component, also implemented as a diffusion model, predicts a sequence of $m$ low-level robot actions, conditioned on the same visual and language features as well as the latent actions.
Conditioning across components is achieved using uni-directional attention over intermediate features, as indicated by the dashed line in Figure~\ref{fig:act}.
Additionally, \texttt{ACT-robot} can incorporate wrist camera input when available.
Unlike prior work~\cite{black2024pi0}, which feeds wrist camera data into the VLM from the start, our design is more computationally efficient.
Another consideration is that we view the wrist camera input as more embodiment-specific and less generalizable, which is why we incorporate it into \texttt{ACT-robot} rather than the VLM.
The first two components, VLM and \texttt{ACT-latent}, are designed to handle the more generalizable aspects of the policy.

One might ask whether the length of the robot action sequence must match that of the latent action sequence, \ie, whether $m = nK$.
In our design, this is not required. We allow different lengths for latent and robot action sequences, as long as they share the same starting time step $t$.
For example, we may model 10 latent actions (corresponding to 20 robot actions if $K=2$) but choose to predict only 4 robot actions (effectively relying on the first 2 latent actions).
This flexibility enables us to maximize the benefits of modeling latent actions.

We highlight three key elements of our design for incorporating latent actions:
\begin{itemize}[nosep, left=10pt]
    \item \textbf{Latent actions as a mid-level bridge.}
    Previous works, including LAPA~\cite{ye2024latent} and GR00T~\cite{nvidia2025gr00t}, treat latent actions similarly to robot actions and do not explicitly model the hierarchical structure between them.
    For example, GR00T simply treats latent actions as an additional action type and trains them alongside robot actions within a shared diffusion transformer.
    In contrast, our model treats latent actions as a distinct mid-level representation that bridges high-level vision and language prompts with low-level robot actions.

    \item \textbf{Explicit transfer from latent to robot actions.}
    Unlike LAPA~\cite{ye2024latent} and GR00T~\cite{nvidia2025gr00t}, where the transfer from latent actions to robot actions occurs only implicitly through pre-trained weight initialization, our model enables an explicit connection.
    The robot action diffusion process is directly conditioned on the latent action diffusion process, allowing more effective and structured information transfer from latent actions to robot actions.
    
    \item \textbf{Modeling latent actions sequences.}
    While prior works (LAPA~\cite{ye2024latent} and GO-1~\cite{agibot-world-contributors2025agibot}
    ) incorporate latent actions, they only model one-step predictions rather than planning over longer horizons at the latent action level.
    In contrast, our approach models a sequence of future latent actions, enabling structured planning at both the latent and robot action levels.
\end{itemize}


\includegraphics[height=8pt]{figs/gear.png} \textbf{Implementation} \quad
We use a pre-trained PaliGemma model~\cite{beyer2024paligemma0} as our VLM.
Both \texttt{ACT-latent} and \texttt{ACT-robot} adopt a transformer architecture following~\cite{zhou2025transfusion0}, and are trained using flow matching~\cite{lipman2022flow,liu2022rectified}.
Wrist camera images are tokenized following the approach used in HPT~\cite{wang2024scaling}.
Similar to the proprio FDM in \lam, we incorporate embodiment context embeddings in \texttt{ACT-robot} to account for embodiment-specific information.
Inspired by Moto~\cite{chen2024moto} and RDT~\cite{liu2024rdt01b0}, we apply attention masking during training: with 50\% probability, we completely disable attention from latent actions to robot actions; otherwise, we randomly mask out attention from 50\% of the latent actions.
Further implementation details are provided in the appendix.

\textnormal{\PaperPortrait}~\textbf{Training, Finetuning and Inference}\quad
During training, we update all components of the model, including both the pre-trained and randomly initialized parts.
The model is trained jointly using losses on both latent actions and robot actions, leveraging a mixture of datasets containing both human video and robot action data including OpenX \cite{open_x_embodiment_rt_x_2023}, Ego4D \cite{Ego4D2022CVPR}, etc.
Finetuning follows the same procedure as training, with the exception that, for unseen embodiments, we initialize a new context embedding.
For robot action inference, we perform denoising steps simultaneously in both \texttt{ACT-Latent} and \texttt{ACT-Robot}. For more details, please refer to Appendix \ref{appA:pi_model}.


==> sections/short_related.tex <==
\section{Related Work}

\paragraph{Visual-Language-Action Models}

Vision-Language-Action (VLA) models~\cite{black2024pi0,li2024cogact,nvidia2025gr00t,chen2024moto,kim2024openvla,zhao2025cot0vla0,xinghang2024vision,open_x_embodiment_rt_x_2023} leverage pre-trained vision-language models (VLMs) to generate robot actions using visual and language cues. They either directly repurpose VLMs for action prediction~\cite{chen2024moto,ye2024latent,xinghang2024vision,kim2024openvla} or use action experts to map VLM outputs to robot actions~\cite{nvidia2025gr00t,black2024pi0,li2024cogact}. While training on large-scale datasets like Open X-Embodiment~\cite{open_x_embodiment_rt_x_2023} enhance the generalization ability of VLAs, cross-embodiment generalization remains challenging due to diverse robot setups and configurations. Utilizing unlabeled trajectory data with pseudo-labels such as latent actions~\cite{ye2024latent,chen2024moto}, language sub-goals~\cite{mu2023embodiedgpt}, or visual sub-goals~\cite{zhao2025cot0vla0} supports overcoming these challenges.
Our method adopts the latent action approach and improves both the modeling of latent actions and their integration into VLA pretraining.

\paragraph{Modeling Latent Actions for VLA Pretraining}

Recent exploration into latent actions began with LAPO~\cite{schmidt2023learning} and Genie~\cite{bruce2024genie}, which primarily focused on the video game domain.
Dynamo~\cite{cui2024dynamo} adopted a similar architecture, using inverse and forward dynamics models to shape state representations.
LAOM~\cite{nikulin2025latentactionlearningrequires} propose to use supervision to learn better latent actions in the presense of distractors on Mujoco environments.

For robotic learning, methods have started to incorporate latent actions into VLA pretraining~\cite{ye2024latent,chen2024igor,chen2024moto,nvidia2025gr00t,agibot-world-contributors2025agibot,bu2025univlalearningacttaskcentric,yang2025comolearningcontinuouslatent, liang2025clam}.
LAPA~\cite{ye2024latent} proposes to learn from videos, and trains its latent actions and Vision-Language Model (VLM) using either human or robot video data.
Concurrently, IGOR~\cite{chen2024igor} learns latent actions from a mixture of human and robot videos, marking the first demonstration of successful latent action transfer between humans and robots in a unified action space for embodied AI.
Moto-GPT~\cite{chen2024moto} co-fine-tunes both latent and robot action labels. GR00T~\cite{nvidia2025gr00t} treats latent actions as a distinct embodiment, while Go-1~\cite{agibot-world-contributors2025agibot} generates robot actions conditioned on discrete latent tokens.
UniVLA~\cite{bu2025univlalearningacttaskcentric} proposes a two-stage training pipeline to learn task-centric latent actions.
More recent works like \cite{yang2025comolearningcontinuouslatent, liang2025clam} explore the continuous latent actions.
By contrast, our approach jointly models latent and robot actions through a joint diffusion process, conditioning robot action generation on latent actions for more effective and structured information transfer.
Our method offers better integration compared to LAPA~\cite{ye2024latent} and GR00T~\cite{nvidia2025gr00t}, incorporates immediate visual context unlike Moto-GPT~\cite{chen2024moto}, and avoids inconsistencies caused by teacher forcing seen in Go-1~\cite{agibot-world-contributors2025agibot}, achieving robust test-time reasoning.

